A First Look at Developers' Live Chat on Gitter

Modern communication platforms such as Gitter and Slack play an increasingly critical role in supporting software teamwork, especially in open source development.Conversations on such platforms often contain intensive, valuable information that may be used for better understanding OSS developer communication and collaboration. However, little work has been done in this regard. To bridge the gap, this paper reports a first comprehensive empirical study on developers' live chat, investigating when they interact, what community structures look like, which topics are discussed, and how they interact. We manually analyze 749 dialogs in the first phase, followed by an automated analysis of over 173K dialogs in the second phase. We find that developers tend to converse more often on weekdays, especially on Wednesdays and Thursdays (UTC), that there are three common community structures observed, that developers tend to discuss topics such as API usages and errors, and that six dialog interaction patterns are identified in the live chat communities. Based on the findings, we provide recommendations for individual developers and OSS communities, highlight desired features for platform vendors, and shed light on future research directions. We believe that the findings and insights will enable a better understanding of developers' live chat, pave the way for other researchers, as well as a better utilization and mining of knowledge embedded in the massive chat history.

==> tab/project1.tex <==
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{table}[tp]
\caption{The statistics of the studied Gitter communities} 
\vspace{-0.3cm}
\label{tab:proj}
\resizebox{\columwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Community}} & \multirow{2}{*}{\textbf{Domain}} & \multicolumn{3}{c|}{\textbf{\tabincell{c}{Entire\\ Population}}} & \multicolumn{3}{c|}{\textbf{\tabincell{c}{Sample\\ Population}}} \\
\cline{3-8}
& &\textbf{P} & \textbf{D} & \textbf{U}& \textbf{P} & \textbf{D} & \textbf{U} \\ \hline
Angular\cite{angular}          & \tabincell{c}{Frontend\\ Framework}         & 22,467                 & 79,619            & 695,183              & 125                       & 97                       &778                         \\ \hline
Appium\cite{appium}           & \tabincell{c}{Mobile\\}                     & 3,979                  & 4,906             & 29,039               & 73                                      & 87                       &724                         \\ \hline
DL4J\cite{deeplearning4j}             & Data Science               & 8,310                  & 27,256            & 252,846              & 93                       & 100                       &1,130                         \\ \hline
Docker\cite{docker}           & DevOps                     & 8,810                  & 3,954             & 22,367               & 74               & 90                       &1,126                         \\ \hline
Ethereum\cite{ethereum}         & \tabincell{c}{Blockchain\\ Platform} & 16,154                 & 17,298            & 91,028               & 116                       & 96                       &516                         \\ \hline
Gitter\cite{gitter}           & \tabincell{c}{Collabration\\ Platform}      & 9,260                  & 7,452             & 34,147               & 87                       & 86                       &515                         \\ \hline
Nodejs\cite{nodejs}           & \tabincell{c}{Web Application\\ Framework}  & 18,118                 & 13,981            & 81,771               & 144                       & 98                       &737                         \\ \hline
Typescript\cite{typescript}       &\tabincell{c}{Programming\\ Language}                   & 8,318                  & 18,812            & 196,513              & 110              & 95                       &1,700                         \\ \hline
\multicolumn{2}{|c|}{\textit{Total}}          & \textit{95,416}        & \textit{173,278}  & \textit{1,402,894}    & \textit{822}             & \textit{749}             &\textit{7,226}               \\ \hline
\end{tabular}

}
\vspace{-0.3cm}
\end{table}

==> tab/taxonomy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}  %表格自动换行
\caption{Beyer's taxonomy\cite{DBLP:conf/iwpc/BeyerM0P18}\todo{larger and lines}}
\label{tab:taxonomy}
 \resizebox{\columnwidth}{!}{
\begin{tabular}{@{}|l|l|@{}}
\hline
\multicolumn{1}{|c|}{Category} & \multicolumn{1}{c|}{Description}                                                                                                                                                                        \\ \hline
API usage                              & Asking for suggestions on how to implement some functionality or how to use an API.                                                                                                                     \\ \hline
Discrepancy                            & About problems and unexpected behavior of code snippets whereas the initiator has no clue how to solve it.                                                                                              \\ \hline
Errors                                 & Asking for help in fixing an error or understanding what the exception means.                                                                                                                           \\ \hline
Review                                & Asking for best practice approaches or ask for help to make decisions, for instance, which API to select.                                                                                               \\ \hline
Conceptual                             & \tabincell{l}{About the limitations of an API and API behavior, as well as about understanding concepts, such as design patterns\\\multicolumn{1}{l}{or architectural styles, and background information about some API.   functionality.}} \\ \hline
API change                             & Questions that arise due to the changes in an API or due to compatibility issues between different versions of an API.                                                                                  \\ \hline
Learning                               & Asking for support to learn on their own.                                                                                                                                                               \\ \hline
\end{tabular}
}
\end{table}

==> tab/taxonomy2.tex <==
% Please add the following required packages to your document preamble:

\begin{table}[b]
\caption{The extended taxonomy of discussion topics based on Beyer's work\cite{DBLP:conf/iwpc/BeyerM0P18}. The two new types are highlighted in bold.}
\label{tab:taxonomy2}
\resizebox{\columnwidth}{!}{
\begin{tabular}{cl}
%\begin{tabular}{@{}p{3pt}p{5pt}@{}}

\toprule
\textbf{Category} &  \multicolumn{1}{c}{\textbf{Description}}                     \\ \midrule
API usage             &\multicolumn{1}{p{8.5cm}}{Asking for suggestions on how to implement some functionality or how to use an API.} \\
Discrepancy             &\multicolumn{1}{p{8.5cm}}{About problems and unexpected behavior of code snippets whereas the initiator has no clue how to solve it.  }                         \\
Errors             &\multicolumn{1}{p{8.5cm}}{Asking for help in fixing an error or understanding what the exception means. }                             \\
Review            &\multicolumn{1}{p{8.5cm}}{Asking for best practice approaches or ask for help to make decisions, for instance, which API to select.} \\
Conceptual            &\multicolumn{1}{p{8.5cm}}{About the limitations of an API and API behavior, as well as about understanding concepts, such as design patterns or architectural styles, and background information about some API functionality.  }      
\\
API change              &\multicolumn{1}{p{8.5cm}}{Questions that arise due to the changes in an API or due to compatibility issues between different versions of an API.}   

\\
\textit{\textbf{General Development}  }           &\multicolumn{1}{p{8.5cm}}{Discussions about general development concerns, such as programming language preference.} 

\\
\textit{\textbf{Social Chatting}}        &\multicolumn{1}{p{8.5cm}}{Discussions that are irrelevant to the technical software development, mainly for leisure or social connection purpose.}   

\\ \bottomrule
\end{tabular}
}
\end{table}
